Multi-Stage Influence Function

Multi-stage training and knowledge transfer, from a large-scale pretraining task to various finetuning tasks, have revolutionized natural language processing and computer vision resulting in state-of-the-art performance improvements. In this paper, we develop a multi-stage influence function score to track predictions from a finetuned model all the way back to the pretraining data. With this score, we can identify the pretraining examples in the pretraining task that contribute most to a prediction in the finetuning task. The proposed multi-stage influence function generalizes the original influence function for a single model in (Koh & Liang, 2017), thereby enabling influence computation through both pretrained and finetuned models. We study two different scenarios with the pretrained embeddings fixed or updated in the finetuning tasks. We test our proposed method in various experiments to show its effectiveness and potential applications.

==> multi-task-learning.tex <==
\section{Multi-task learning setting}
If we use a multi-task learning setting to minimize the loss on pretrain and finetune data simultaneously while two tasks shares the same embedding weights $W$, we have
\begin{equation}
        \hat{W}_{\epsilon},\hat{U}_{\epsilon},\hat{\Theta}_\epsilon = \argmin_{W,U,\Theta} \lambda F(W,\Theta)+G(W,U) + \epsilon g(z, W, U),
\end{equation}
where $\lambda$ is a constant balancing the pretrain and finetune tasks' losses. The first order condition gives
\begin{equation} 
\begin{split}
\lambda\frac{\partial F}{\partial W} +\frac{\partial G}{\partial W}+\epsilon\frac{\partial g}{\partial W}& = 0 \\
\lambda\frac{\partial F}{\partial \Theta} & = 0 \\
\frac{\partial G}{\partial U}+\epsilon\frac{\partial g}{\partial U}& = 0 \\
\end{split}
\end{equation}
Taking $\epsilon=0$ and the total derivatives give
\begin{equation} 
\begin{split}
(\lambda\frac{\partial^2 F}{\partial W^2}+\frac{\partial^2 G}{\partial W^2})dW + \lambda\frac{\partial^2 F}{\partial W\partial \Theta}d\Theta+\frac{\partial^2 G}{\partial U^2}dU& = -\frac{\partial g}{\partial W}d\epsilon \\
\lambda\frac{\partial^2 F}{\partial W\partial \Theta}dW+\lambda\frac{\partial^2 F}{\partial \Theta^2}d\Theta& = 0 \\
\frac{\partial^2 G}{\partial W\partial U}dW+\frac{\partial^2 G}{\partial U^2}dU& = -\frac{\partial g}{\partial U}d\epsilon 
\end{split}
\end{equation}
So we have
\begin{equation} 
\begin{bmatrix}
\frac{dW}{d\epsilon} \\ \frac{d\Theta}{d\epsilon} \\ \frac{dU}{d\epsilon}
\end{bmatrix}=-
\begin{bmatrix}
\lambda\frac{\partial^2 F}{\partial W^2}+\frac{\partial^2 G}{\partial W^2} & \lambda\frac{\partial^2 F}{\partial W\partial \Theta} & \frac{\partial^2 G}{\partial U^2} \\
\frac{\partial^2 F}{\partial W\partial \Theta} & \frac{\partial^2 F}{\partial \Theta^2} & 0 \\
\frac{\partial^2 G}{\partial W\partial U} & 0& \frac{\partial^2 G}{\partial U^2}
\end{bmatrix}^{-1}
\begin{bmatrix}
\frac{\partial g}{\partial W} \\ 0 \\ \frac{\partial g}{\partial U} 
\end{bmatrix},
\end{equation}
which is entangled with two Hessians and is very hard to compute using only HVP.


